LoD-Loc v3: Generalized Aerial Localization in Dense Cities using Instance Silhouette Alignment

We present LoD-Loc v3, a novel method for generalized aerial visual localization in dense urban environments. While prior work LoD-Loc v2 achieves localization through semantic building silhouette alignment with low-detail city models, it suffers from two key limitations: poor cross-scene generalization and frequent failure in dense building scenes. Our method addresses these challenges through two key innovations. First, we develop a new synthetic data generation pipeline that produces InsLoD-Loc - the largest instance segmentation dataset for aerial imagery to date, comprising 100k images with precise instance building annotations. This enables trained models to exhibit remarkable zero-shot generalization capability. Second, we reformulate the localization paradigm by shifting from semantic to instance silhouette alignment, which significantly reduces pose estimation ambiguity in dense scenes. Extensive experiments demonstrate that LoD-Loc v3 outperforms existing state-of-the-art (SOTA) baselines, achieving superior performance in both cross-scene and dense urban scenarios with a large margin. The project is available at https://nudt-sawlab.github.io/LoD-Locv3/.

==> Tab/ablation_study_2.tex <==
\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{2.8pt} % 调整列间距
\begin{tabular}{ccccccccccccc} 
\toprule
\multirow{2}{*}{Method} & \multicolumn{4}{c}{\textit{Japan\_02}}   & \multicolumn{4}{c}{\textit{Japan\_06}} & \multicolumn{4}{c}{\textit{Japan\_07}}  \\ 
\cmidrule(r){2-5} \cmidrule(r){6-9} \cmidrule(r){10-13}
                        & 2m-2$^\circ$ & 3m-3° & 5m-5° & T.e./R.e. & 2m-2° & 3m-3° & 5m-5° & T.e./R.e.      & 2m-2° & 3m-3° & 5m-5° & T.e./R.e.       \\ 
\cmidrule(r){1-13}
LoD-Loc v2             & 15.60        & 33.80 & 62.40 & 4.05/0.36 & 17.20 & 38.10 & 66.80 & 3.70/0.36      & 21.80 & 42.60 & 73.00 & 3.45/0.36       \\
\textbf{LoD-Loc v3}     & \textbf{33.70}        & \textbf{59.90} & \textbf{87.00} & \textbf{2.24/0.25} & \textbf{36.30} & \textbf{65.40} & \textbf{90.30} & \textbf{2.11/0.25}      & \textbf{37.90} & \textbf{63.60} & \textbf{82.90} & \textbf{2.09/0.25}       \\
\hline
\end{tabular}
% \caption{\textbf{Quantitative comparison of different methods under identical training protocols on the Tokyo-LoDv3 datasets.} The results demonstrate that the superior generalization of our method is not merely a product of high-quality training data, but is fundamentally attributable to our proposed instance alignment mechanism.}
\caption{\textbf{Quantitative comparison of different methods on the Tokyo-LoDv3 dataset under the same training set.} Compared to LoD-Loc v2, our method significantly improves visual localization performance in dense urban scenes.}
\label{Tab:ablation_2}
\end{table*}

==> Tab/rain_localization.tex <==
% \begin{table}
% \setlength{\tabcolsep}{1.8pt} % 调整列间距
% \centering
% \begin{tabular}{cccccc} 
% \toprule
% Dataset                     & Method              & 2m-2$^\circ$ & 3m-3° & 5m-5° & T.e./R.e.           \\ 
% \hline
% \multirow{2}{*}{Japan\_09*} & LoD-Loc v2          & 1.80         & 3.10  & 8.70  & 14.69/0.99          \\
%                             & \textbf{LoD-Loc v3} & 24.70        & 55.10 & 93.70 & 2.86\textbf{/}0.23  \\
% \toprule
% \end{tabular}
% % \caption{\textbf{Quantitative comparison of different methods under identical training protocols on the UAVD4L-LoDv2 and Swiss-EPFLv2 datasets.} The results demonstrate that the superior generalization of our method is not merely a product of high-quality training data, but is fundamentally attributable to our proposed instance alignment mechanism.}
% % \label{Tab:adverse_weather_results}
% \end{table}

\begin{table}[htbp]
\centering
\begin{tabular}{ccccc} 
\toprule
\multirow{2}{*}{Method} & \multicolumn{4}{c}{\textit{Japan\_09*}}                     \\ 
\cmidrule(r){2-5}
                        & 2m-2$^\circ$ & 3m-3° & 5m-5° & T.e./R.e.           \\ 
\cmidrule(r){1-5}
LoD-Loc v2              & 1.80         & 3.10  & 8.70  & 14.69/0.99          \\
\textbf{LoD-Loc v3}     & 24.70        & 55.10 & 93.70 & 2.86\textbf{/}0.23  \\
\toprule
\end{tabular}
\caption{Localization performance of our method.}
\label{Tab:adverse_weather_results}
\end{table}
